Functorial Semantics for Relational Theories

We introduce the concept of Frobenius theory as a generalisation of Lawvere's functorial semantics approach to categorical universal algebra. Whereas the universe for models of Lawvere theories is the category of sets and functions, or more generally cartesian categories, Frobenius theories take their models in the category of sets and relations, or more generally in cartesian bicategories.

==> graffles/macro.tex <==
\newcommand{\cgr}[2][scale=0.45]{\raisebox{0.1em}{\begingroup
\setbox0=\hbox{\includegraphics[#1]{graffles/#2}}%
\parbox{\wd0}{\box0}\endgroup}} 





\newcommand{\dup}{\Delta}
\newcommand{\dis}{!}

\newcommand{\codup}{\nabla}
\newcommand{\codis}{?}
\newcommand{\Frob}[1]{ Frob_{#1} }





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           %
%  Thesis Macros                                            %
%                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\DeclareMathOperator{\Cmp}{Cmp}

\DeclareMathOperator{\Cmp}{\mathbf{Cmp}}
%\DeclareMathOperator{\Psd}{Psd}
%\DeclareMathOperator{\Cospan}{Cospan}
%\DeclareMathOperator{\Cospani}{Cospan^{\cong}}
\DeclareMathOperator{\ILC}{ILC}
\DeclareMathOperator{\OLC}{OLC}
\DeclareMathOperator{\LC}{LC}
\DeclareMathOperator{\Psd}{\mathbf{Psd}}
\DeclareMathOperator{\PsdCocone}{\mathbf{PsdCocone}}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\ke}{ker}
%\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Spl}{Spl}
\DeclareMathOperator{\op}{op}
\DeclareMathOperator{\Ob}{ob}
\DeclareMathOperator{\Arr}{arr}
\DeclareMathOperator{\Cel}{cel}
\DeclareMathOperator{\Sh}{Sh}
\DeclareMathOperator{\germ}{germ}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\tw}{\mathit{tw}}
\DeclareMathOperator{\Nil}{Nil}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\Deck}{Deck}
\DeclareMathOperator{\Conn}{Conn}
\DeclareMathOperator{\Th}{\mathsf{Th}}
\DeclareMathOperator{\TTh}{\mathsf{2-Th}}
\DeclareMathOperator{\Root}{rt}
\DeclareMathOperator{\Char}{ch}
%\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\Bicolim}{Bic}
\DeclareMathOperator{\RBC}{RBC}
\DeclareMathOperator{\LTS}{LTS}
\DeclareMathOperator{\GLTS}{ATS}
\DeclareMathOperator{\CTS}{CTS}
\DeclareMathOperator{\SEW}{Sew}
\DeclareMathOperator{\FLTS}{FLTS}
\DeclareMathOperator{\STS}{STS}
%\DeclareMathOperator{\Rel}{Rel}

\renewcommand{\P}{\mathcal{P}}
\newcommand{\eg}{\textit{e.g.\ }}
\newcommand{\cf}{\textit{cf.\ }}
\newcommand{\fig}[1]{{\textit{Fig.~}{#1}}}

\newcommand{\leakOut}[1]{\uparrow\!#1}
\newcommand{\leakIn}[1]{\downarrow\!#1}
\newcommand{\typedState}[2]{{\scriptstyle \left<#1\,|\,#2\right>}}
\newcommand{\Defeq}% definitional equality
 {\stackrel{\mathrm{def}}{=}}

\newcommand{\ctx}{\mathcal{C}}
\newcommand{\evCtx}{\mathcal{E}}
\newcommand{\nEvCtx}{\mathcal{X}}
\newcommand{\strCong}{\equiv}
\newcommand{\nStrCong}{\nequiv}
\newcommand{\rel}[1]{\mathrel{\mathcal{#1}}}

\newcommand{\sLambdaBind}[2]{\boldsymbol{\lambda} #1.\,#2}
\newcommand{\lambdaBind}[2]{\lambda #1.\,#2}
\newcommand{\reduction}{\,\rightarrow\,}
\newcommand{\mReduction}{\,\rightarrow^*\,}
\newcommand{\xRightarrow}[1]{\stackrel{#1}{\Rightarrow}}
\newcommand{\weakLabelledTransition}[1]{{\,\xRightarrow{#1}\,}}
\newcommand{\labelledTransition}[1]{{\,\xrightarrow{#1}\,}}
\newcommand{\derivationRule}[3]{{\prooftree{\scriptstyle #1}\justifies{\scriptstyle #2}\using\ruleLabel{#3}\endprooftree}}
\newcommand{\reductionRule}[2]{{\prooftree{\scriptstyle #1}\justifies{\scriptstyle #2}\endprooftree}}

\newcommand{\barbson}[1]{\!\downarrow_{#1}}
\newcommand{\weakbarbson}[1]{\!\Downarrow_{#1}}
 
\newcommand{\fresh}{\mathit{fr}}

\newcommand{\ent}{\vdash}
\newcommand{\typ}{\mathrel{:}}
\newcommand{\judgement}[2]{#1\;\vdash\;#2}


\newcommand{\outputPrefix}[2]{{#1}!{#2}}
\newcommand{\inputPrefix}[2]{{#1}?{#2}}
\newcommand{\outputLabel}[1]{{#1}!}
\newcommand{\inputLabel}[1]{{#1}?}
\newcommand{\leakLabel}[1]{{\##1}}
\newcommand{\boundOutput}[2]{{#1}!{(#2)}}

\newcommand{\transitionSpace}{\phantom{P\xsta{a}Q}}

\newcommand{\Input}{\mathscr{I}}
\newcommand{\Output}{\mathscr{O}}
\newcommand{\Process}{\mathscr{P}}
\newcommand{\Name}{\mathscr{N}}

\newcommand{\calc}{$\epsilon$cs}
\newcommand{\stran}{\raise1pt\hbox{$\centerdot$}}
\newcommand{\SEWC}{\SEW^{c}}

\newcommand{\ruleLabel}[1]{\textsc{\scriptsize{(#1)}}}
\newcommand{\ruleName}[1]{\ruleLabel{#1}}

\newcommand{\rring}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\field}[1]{\ensuremath{\mathbf{#1}}}
\renewcommand{\b}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Z}{\rring{Z}}

%\newcommand{\C}{\rring{C}}

\newcommand{\R}{\rring{R}}

\newcommand{\Q}{\rring{Q}}

\newcommand{\N}{\rring{N}}

%\newcommand{\T}{\rring{T}}

\renewcommand{\k}{\field{k}}

\newcommand{\K}{\field{K}} 

\newcommand{\CF}{\mathcal{C}}

\newcommand{\fg}[1]{\pi_{1}(#1)}

\newcommand{\setn}[2]{\{\,{#1}\,\mid\,{#2}\,\}}

\newcommand{\pres}[2]{<\,#1\ |\ #2\,>} 

\newcommand{\s}[2]{\stackrel{#1}{#2}}

\newcommand{\cm}{\circ}

\newcommand{\ra}{\to}

\newcommand{\la}{\gets}

\newcommand{\rra}{\rightrightarrows}

\newcommand{\lra}{\longrightarrow}

\newcommand{\Ra}{\Rightarrow}

\newcommand{\lmt}{\longmapsto}

\newcommand{\ob}[1]{\overline{#1}}

\newcommand{\rad}{\text{r}}

\newcommand{\ten}{\otimes}

\newcommand{\dsum}{\oplus}

\newcommand{\ds}{\oplus}

\newcommand{\iso}{\cong}

\newcommand{\Alg}[1]{#1\text{-}\cat{Alg}}
\newcommand{\Mod}[1]{#1\text{-}\cat{Mod}}
\newcommand{\kAlg}{\Alg{k}}
\newcommand{\KAlg}{\Alg{K}}
\newcommand{\kMod}{\Mod{k}}
\newcommand{\KMod}{\Mod{K}}
\newcommand{\TAlg}{\Alg{T}}
\newcommand{\CRng}{\cat{CRng}}
\newcommand{\Grp}{\cat{Grp}}
\newcommand{\Ab}{\cat{Ab}}
\newcommand{\al}{\alpha}
\newcommand{\Set}{\cat{Set}}
\newcommand{\Rel}{\cat{Rel}}
\newcommand{\Cat}{\cat{Cat}}
\newcommand{\Par}{\cat{Par}}
\newcommand{\Prl}{\cat{Prl}}
\newcommand{\GCat}{G\textrm{-}\cat{Cat}\xspace}
%\newcommand{\Top}{\cat{Top}}
\newcommand{\Topp}{\cat{Top_*}}
\newcommand{\Graph}{\cat{Graph}\xspace}
\newcommand{\Bun}{\cat{Bun}\xspace}
\newcommand{\ABun}{\cat{ABun}\xspace}
\newcommand{\Ord}{\cat{Ord}\xspace}

\newcommand{\CC}{\cat{C}\xspace}

\newcommand{\DD}{\cat{D}\xspace}

\newcommand{\EE}{\cat{E}\xspace}

\newcommand{\XX}{\cat{X}\xspace}



\newcommand{\SubZ}{\text{Sub($Z$)}\xspace}
\newcommand{\Sub}[1]{\text{Sub(${#1}$)}}
\newcommand{\Desp}{\text{Des($p$)}\xspace}



\newcommand{\diag}{\Delta}

\newcommand{\codiag}{\triangledown}

\newcommand{\LH}{\cat{LH}}

\newcommand{\emb}{\hookrightarrow}

\newcommand{\scr}[1]{\mathscr{#1}}

\renewcommand{\O}{\boldsymbol{\mathcal{O}}}
\renewcommand{\emptyset}{\varnothing}

\renewcommand{\c}{\cdot}
\renewcommand{\t}{\times}

\renewcommand{\binom}[2]{\left(\begin{smallmatrix} #1 \\ #2 \end{smallmatrix}\right)}

\newcommand{\trinom}[3]{\left(\begin{smallmatrix} #1 \\ #2 \\  #3 \end{smallmatrix}\right)}



\newcommand{\ladj}[2]{\ar@/^/[#1]^-{#2} \ar@{}[#1]|-%

{\ifthenelse{\equal{#1}{r}}{\bot}{%

{\ifthenelse{\equal{#1}{rr}}{\bot}{%

{\ifthenelse{\equal{#1}{l}}{\top}{%

{\ifthenelse{\equal{#1}{u}}{\dashv}{%

{\vdash}}}}}}}}}}



\newcommand{\radj}[2]{\ar@/^/[#1]^-{#2}}

\newcommand{\radjff}[2]{\ar@{_{(}->}[#1]^{#2}}

\newcommand{\pullbacktop}[4]{%

{#1} \ar@/_/[ddr]_{#4} \ar@/^/[drr]^{#2}% 

\ar@{.>}[dr]|-{#3} \\}

\newcommand{\pullbackbot}[8]{%

& {#1} \ar[r]^{#2} \ar[d]^{#3} & {#4} \ar[d]^{#5} \\%

& {#6}  \ar[r]_{#7}  & {#8}}


\newtheorem{clm}{Claim}[section]
\newtheorem{cor}[clm]{Corollary}
\newtheorem{pro}[clm]{Proposition}
\newtheorem{defn}[clm]{Definition}
\newtheorem{lem}[clm]{Lemma}
\newtheorem{thm}[clm]{Theorem}
\newtheorem{sch}[clm]{Scholium}
\newtheorem{exm}[clm]{Example}
\newtheorem{cexm}[clm]{Counterexample}
\newtheorem{alg}[clm]{Algorithm}
\newtheorem{rmk}[clm]{Remark}
\newtheorem{exr}[clm]{Exercise}

\newcommand{\fancy}[1]{\mathbf{#1}}

\newcommand{\cat}[1]{\mathbf{#1}}
\newcommand{\precat}[1]{\ensuremath{\,{\acute{}}\mathbf{#1}}}

\newcommand{\catlim}{\varprojlim}

\newcommand{\catcolim}{\varinjlim}

%\newcommand{\xra}[1]{\xrightarrow{#1}}

\newcommand{\xra}[1]{\stackrel{#1}{\longrightarrow}}

%\newcommand{\xla}[1]{\xleftarrow{#1}}

\newcommand{\xla}[1]{\stackrel{#1}{\longleftarrow}}

\newcommand{\wt}[1]{\widetilde{#1}}

\newcommand{\wh}[1]{\widehat{#1}}

\newcommand{\equ}{\simeq}



\newcommand{\bsigma}{{\boldsymbol{\sigma}}}

\newcommand{\btau}{{\boldsymbol{\tau}}}

\newcommand{\biota}{{\boldsymbol{\iota}}}

\newcommand{\tuple}[1]{\left\langle {#1} \right\rangle}

\newcommand{\hra}{\hookrightarrow}

\newcommand{\smallxy}{\def\objectstyle{\scriptstyle}\def\labelstyle{\scriptstyle}}

\newcommand{\sm}[1]{\hbox{\tiny{$#1$}}}

%\newcommand{\Xsta}[1]{\stackrel{#1}{%
% \rlap{\rule[2.8pt]{1.5em}{0.3pt}}%
% \rule[0.8pt]{1.5em}{0.3pt}%
%\mkern-6mu\blacktriangleright}}

\newcommand{\xsta}[1]{\hbox{$\,\stackrel{\,#1}{\rule[2.2pt]{1.0em}{0.6pt}}%
\mkern-2mu\blacktriangleright\,$}}
\newcommand{\lxsta}[1]{\hbox{$\,\stackrel{#1}{\rule[2.2pt]{1.5em}{0.6pt}}\mkern-2mu\blacktriangleright\,$}}
\newcommand{\longxsta}[1]{\hbox{$\,\stackrel{#1}{\rule[2.2pt]{2.5em}{0.6pt}}%
\mkern-2mu\blacktriangleright\,$}}
\newcommand{\superlongxsta}[1]{\hbox{$\,\stackrel{#1}{\rule[2.2pt]{3.5em}{0.6pt}}%
\mkern-2mu\blacktriangleright\,$}}
\newcommand{\superduperlongxsta}[1]{\hbox{$\,\stackrel{#1}{\rule[2.2pt]{4.5em}{0.6pt}}%
\mkern-2mu\blacktriangleright\,$}}

\newcommand{\nrta}{\hbox{$\,\mathrel{\rule[2.2pt]{1.5em}{0.6pt}}%
\mkern-2mu\not\vartriangleright\,$}}
\newcommand{\rta}{\hbox{$\,\mathrel{\rule[2.2pt]{1.5em}{0.6pt}}%
\mkern-2mu\vartriangleright\,$}}
\newcommand{\sta}{\hbox{$\,\mathrel{\rule[2.2pt]{1.5em}{0.6pt}}%
\mkern-2mu\blacktriangleright\,$}}

\newcommand{\hco}{\circ}
\newcommand{\vco}{\,{\scriptstyle\bullet}\,}

\newcommand{\mmid}{\mathrel{\boldsymbol\mid}}
\newcommand{\zero}{\mathtt{0}}

\newenvironment{funnyMathDisp}{\par\noindent\rule\textwidth{0.8pt}%
\vskip-9pt\noindent\rule\textwidth{0.4pt}\[}
{\]\rule\textwidth{0.4pt}\vskip-9pt%

\noindent\rule\textwidth{0.8pt}\vskip\belowdisplayskip\noindent}


\let\from\colon

\newcommand\red{\mathit{red}}

\newcommand\blue{\mathit{blue}}

\newcommand\tra{\lesssim_{\mathrm{tr}}}

\newcommand\fail{\lesssim_{\mathrm{f}}}

\newcommand{\PB}{{\sf Pb}\xspace}

\newcommand{\PO}{{\sf Po}\xspace}

\newcounter{ncomm}
\newcommand{\olds}[1]{\oldstylenums{#1}}
\newcommand{\oldsb}[1]{{\bfseries\olds{#1}}}
\newcommand{\comment}[1]{\stepcounter{ncomm}%
\vbox to0pt{\vss\llap{\tiny\oldsb{\arabic{ncomm}}}\vskip6pt}%
\marginpar{\tiny\bf\raggedright%
{\oldsb{\arabic{ncomm}}}.\hskip0.5em#1}}

\newcommand{\ltsred}[1]
{ \setbox0=\hbox{$\ {}^{#1}\ $}
  \setbox1=\hbox{$\longrightarrow$}
  \loop\setbox1=\hbox{$-$\kern-0.3em\unhbox1}\ifdim\wd1<\wd0\repeat
  \hbox{$\ \ \mathop{\box1}\limits^{#1}\ \ $}
}

\newcommand{\arx}[2]{\!\xymatrix@=15pt{\ar[r]^{{#1}}_{{#2}}&}\!}

\newcommand{\Rar}{\Rightarrow}

\newcommand{\react}[1]{\mathbb{#1}}

\newcommand{\ehole}{0}

\newcommand{\ass}{a}

\newlength{\mylength}

\newenvironment{Framed}% 
{\setlength{\fboxsep}{15pt} 
\setlength{\mylength}{\linewidth}% 
\addtolength{\mylength}{-2\fboxsep}% 
\addtolength{\mylength}{-2\fboxrule}% 
\Sbox 
\minipage{\mylength}% 
\setlength{\abovedisplayskip}{0pt}% 
\setlength{\belowdisplayskip}{0pt}% 
}% 
{\endminipage\endSbox 
\[\fbox{\TheSbox}\]}

\newcommand{\bnfSep}{\ |\ }
\newcommand{\bnfEq}{\ ::=\ }




\usepackage[english]{babel}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
%\usepackage[utf8]{inputenc}
%\usepackage[T1,T2A]{fontenc}
%\usepackage[T1]{fontenc}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx,epsfig,color}
\usepackage[color]{xypic}
\xyoption{rotate}
\input xy
\xyoption{all}
\xyoption{2cell}
\UseAllTwocells
\usepackage{comment}
\usepackage{etoolbox}
\usepackage{multicol}
%% MACROS FOR ELSEVIER CLASS^%%%

%
% Theorem environments
%
%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}[theorem]{Example}
\newtheorem{exams}[theorem]{Examples}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{opro}[theorem]{Open Problem}
\newtheorem{obser}[theorem]{Observation}
\newtheorem{constr}[theorem]{Construction}
\newtheorem{remark}[theorem]{Remark}

%\newproof{proof}{Proof}

% MARGIN COMMENTS
%\usepackage[layout=margin,draft]{fixme}
\usepackage[layout=margin]{fixme}

%
% FIXME setup
%
\FXRegisterAuthor{fz}{afz}{Fab}%Fabio
\FXRegisterAuthor{ps}{aps}{Chavez}%Pawel
\FXRegisterAuthor{fb}{afb}{Trotski}%Filippo

\newcommand{\pippo}[1]{\fbnote{ #1 }}    % Commento a lato, Filippo
\newcommand{\fabio}[1]{\fznote{ #1 }}    % Commento a lato, Fabio
\newcommand{\pawel}[1]{\psnote{ #1 }}    % Commento a lato, Pawel
% RIMOSSI PER SOTTOMISSIONE
%\newcommand{\pippo}[1]{}    % Commento a lato, Filippo
%\newcommand{\fabio}[1]{}    % Commento a lato, Fabio
%\newcommand{\pawel}[1]{}    % Commento a lato, Pawel

\newcommand \xmapsto[1] {\overset{#1}{\mapsto}}
\newcommand\starredtext[2]{\begin{center}\parbox{8.6cm}{#1}\hspace*{1.5cm}(#2)\end{center}}

\newcommand{\pullbackcorner}[1][d]{\save*!/#1+1.0pc/#1:(1,-1)@^{|-}\restore}
\newcommand{\pushoutcorner}[1][d]{\save*!/#1-1.0pc/#1:(-1,1)@^{|-}\restore}



\newcommand{\bb}[1]{\ensuremath{[\![{#1}]\!]}}

\def \df {\ \ensuremath{:=}\ }
\def \To {\Rightarrow}
\def \dfop {\ \ensuremath{=\!\!:}\ }
\def \tns {\oplus}
\def \: {\colon}
\def \poi {\,\ensuremath{;}\,}
\newcommand\bicomp[1] {\hspace{-.2pt}{\otimes}_{\scriptscriptstyle #1}\hspace{-.2pt}}%{\mf{C}}
\newcommand\compP {\poi}% comp of PROPs
\newcommand{\eql}[1]{\ \overset{\text{#1}}=\ }
\newcommand{\tr}[1]{\xrightarrow{#1}}    % --1-->
\newcommand{\tl}[1]{\xleftarrow{#1}}    % <--1--


\newcommand\funF{\mathcal{F}}
\newcommand\G{\mathcal{G}}
\newcommand\FH{\mathcal{H}}
\newcommand\FM{\mathcal{M}}
%\newcommand\id{\mathit{id}}
%\newcommand{\op}[1]{#1^{\scriptstyle \mathit{op}}}
\def \N {\mathbb{N}}
\def \catC {\mathbb{C}}%{\mf{C}}
\def \Perm {\mathsf{P}} %{\mf{P}}
\def \Set {\mathbf{Set}}% Set
\def \Cat {\mathbf{Cat}}% CAT
\def \F {\mathsf{F}}
\def \Fop {\op{\F}}
\def \PROP {\mathbf{PROP}} % category of PROPs
\def \PRO {\mathbf{PRO}} % category of PROs
\newcommand\T{\mathcal{T}} % arbitrary PROP
\def \PS {\mathsf{S}} % arbitrary PROP
\def \Mon {\mathsf{Mn}}  % PRO of monoids
\def \Com {\mathsf{Cm}} % PRO of comonoids
\def \CMon {\mathsf{CMn}} % PROP of commutative monoids
\def \CCom {\mathsf{CCm}} % PROP of commutative comonoids
\def \frob {\mathsf{Frob}}

\newcommand{\SB}{\mathsf{SB}} % prop of special bialgebras
 \newcommand{\B}{\mathsf{B}}  % prop of bialgebras
 \newcommand{\Inj}{\mathsf{In}}  % the prop of injections
\newcommand{\Surj}{\mathsf{Su}} % the prop of surjections
\newcommand{\Span}[1]{\mathsf{Span}(#1)}
\newcommand{\Cospan}[1]{\mathsf{Cospan}(#1)}
\usepackage{bbm}
  \def \UNIT {\mathsf{Un}} % the prop of unit
   \def \MULT {\mathsf{Mu}} % the prop of mult
  %\def \UNIT {\mathbb{U}} % the prop of unit
   %\def \MULT {\mathbb{M}\mathbbm{u}} % the prop of mult

\def\lambdapb {\lambda_{\scriptscriptstyle \mathit{pb}}}
\def\lambdapo {\lambda_{\scriptscriptstyle \mathit{po}}}



\newcommand\ord[1] {\overline{#1}}

\newcommand \LwA[1] {\mathcal{L}_{\scriptscriptstyle #1}}
\newcommand \Lw {\LwA{}}
\newcommand \var[1] {\mathit{ovar}(#1)}
\newcommand \size[1] {|#1|}
\newcommand\OpDiag{\lower4pt\hbox{$\includegraphics[width=24pt]{graffles/OpDiag.pdf}$}}
\newcommand\diagD{\lower4pt\hbox{$\includegraphics[width=24pt]{graffles/diagD.pdf}$}}
\newcommand \tpl[1] {{\langle#1\rangle}} %tuple
\newcommand \Mquot {\theta} % monad quotient
\def \bicat {\mathfrak{B}}
\newcommand{\model}[1]{\mathsf{LinMod}(#1)} % models of a PRO
\newcommand{\Prof}[1]{\mathsf{Prof}(#1)}
\newcommand{\MonC}{\mathbf{Mon}} % category of monoids
\newcommand \copia[1] {\mathit{cpy}(#1)}
\newcommand \discard[1] {\mathit{dsc}(#1)}
\newcommand{\LawMod}[1]{\mathsf{CartMod}(#1)} % models of a Lawvere theory
\newcommand{\modelPROP}[1]{\mathsf{SLinMod}(#1)} % models of a PROP
\def \catD {\mathbb{D}}%{\mf{C}}
\def \catE {\mathbb{E}}%{\mf{C}}
\newcommand{\Ar}[1]{\mathit{Ar}_{\scriptscriptstyle #1}}
%\newcommand{\Ob}[1]{\mathit{Ob}_{\scriptscriptstyle #1}}
\newcommand{\ObO}{\Ob{}}
\newcommand{\ArO}{\Ar{}}
\newcommand{\dom}[1]{\mathit{dom}_{\scriptscriptstyle #1}}
\newcommand{\cod}[1]{\mathit{cod}_{\scriptscriptstyle #1}}
\newcommand{\domO}{\dom{}}
\newcommand{\codO}{\cod{}}
%\newcommand{\Mod}[1]{\mathsf{Bimod}(#1)} % bicategory of bimodules
\newcommand{\ComToLw}{\Phi} % inclusion of Com in Lw
\newcommand{\FreePToLw}{\Psi} % inclusion of free PROP in Lw
\newcommand{\freeP}[1]{\T_{\scriptscriptstyle #1}} % free PROP

\newcommand{\freePRO}[1]{\PS_{\scriptscriptstyle #1}} % free PRO



\newcommand\Idnet{\lower3pt\hbox{$\includegraphics[width=20pt]{graffles/id.pdf}$}}
\newcommand\symNet{\lower3pt\hbox{$\includegraphics[width=20pt]{graffles/symmetryalt.pdf}$}}
\newcommand{\ZeronetT}{\lower4pt\hbox{$\includegraphics[width=14pt]{graffles/idzerocircuit.pdf}$}}


\newcommand\Bmult{\lower5pt\hbox{$\includegraphics[width=20pt]{graffles/Bmult.pdf}$}}
\newcommand\Bcomult{\lower5pt\hbox{$\includegraphics[width=20pt]{graffles/Bcomult.pdf}$}}
\newcommand\Bunit{\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/Bunit.pdf}$}}
\newcommand\Bcounit{\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/Bcounit.pdf}$}}

\newcommand\Wmult{\lower5pt\hbox{$\includegraphics[width=20pt]{graffles/Wmult.pdf}$}}
\newcommand\Wcomult{\lower5pt\hbox{$\includegraphics[width=20pt]{graffles/Wcomult.pdf}$}}
\newcommand\Wunit{\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/Wunit.pdf}$}}
\newcommand\Wcounit{\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/Wcounit.pdf}$}}

\newcommand\twoBcounit{\lower5pt\hbox{$\includegraphics[width=15pt]{graffles/lunitsr.pdf}$}}




